dMX: Differentiable Mixed-Precision Assignment for Low-Precision Floating-Point Formats

Quantizing large language models (LLMs) to low-precision floating-point representations is central to efficient deployment, yet applying a single bit-width uniformly across all layers is sub-optimal in terms of both performance and accuracy. This work introduces dMX, a differentiable mixed-precision quantization framework for learnable floating-point bit-width assignment. We study its application for the microscaling floating-point (MXFP) family of data types defined by the Open Compute Project (OCP) standard. The per-layer bit-width assignment is formulated as a continuous optimization problem in which each layer's floating-point format format is parameterized by a scalar parameter, folding the multi-variate design space into a single learnable offset. During training this offset takes continuous values, avoiding sudden oscillations between discrete quantization formats. A temperature-based annealing schedule progressively discretizes the learned offsets, ensuring that the final configuration maps to hardware-compatible MXFP formats without abrupt transitions between training and inference behavior. A target-aware regularization term steers the average bit-width toward a user-specified budget, serving as a coarse-grained proxy for inference cost and balancing model quality against deployment efficiency. We performed experiments on different families of LLM, such as Llama, Qwen3, and SmolLM2, evaluating perplexity on WikiText-2 and accuracy on four zero-shot reasoning benchmarks. Across these settings, dMX consistently yields Pareto-dominating models and improves over Kullback-Leibler (KL) divergence-based layer-selection heuristics, efficiently navigating trade-offs between model quality and average bit-width.

==> images/frequency_heatmap.tex <==
% Per-tensor / per-layer high-precision-frequency heatmap (pgfplots version)
%
% Reproduces a score-heatmap-style figure: rows are tensor (projection) types,
% columns are decoder-layer indices, and each cell is coloured by the fraction
% of mixed-precision configurations in which that layer was kept at the
% high-precision format (viridis sequential colormap, fixed 0..1 scale).
%
% =====================================================================
% HOW TO USE
% =====================================================================
% Define the parameter macros with \def, then \input this file.
% You can \input this file multiple times with different parameters.
%
%   \def\heatmapcsv{images/frequency_mxfp8/meta-llama__Llama-3.1-8B.csv}
%   \def\heatmaptitle{Llama-3.1-8B}
%   \input{images/frequency_heatmap.tex}
%
% Or use the defaults wrapper:
%   \input{images/frequency_heatmap_llama.tex}
%
% =====================================================================
% REQUIRED PREAMBLE (already present in main.tex)
% =====================================================================
%   \usepackage{xcolor}
%   \usepackage{pgfplots}
%   \usepackage{pgfplotstable}
%   \pgfplotsset{compat=1.18}
%
% =====================================================================
% PARAMETERS (must be defined before \input)
% =====================================================================
%   \heatmapcsv    — CSV file path (relative to the compiling .tex root)
%   \heatmaptitle  — plot title (model name)
%   \heatmapnlayers— number of decoder layers (columns).  Optional; defaults
%                    to 32.  E.g. \def\heatmapnlayers{16} for Llama-3.2-1B.
%
% =====================================================================
% CSV FORMAT
% =====================================================================
%   layer,high_precision_frequency
%
%   - layer                     : <tensor-type>_<decoder-layer-index>,
%                                 e.g. gate_proj_31
%   - high_precision_frequency  : fraction in [0,1]
%
% Recognised tensor types (rows, top -> bottom):
%   q_proj, k_proj, v_proj, o_proj, gate_proj, up_proj, down_proj
% Decoder-layer index runs 0..31.
% =====================================================================

% ----- viridis sequential colormap (dark blue/purple -> green -> yellow) ----
% Defined inline (idempotently) so the file does not depend on the pgfplots
% "colormaps" library.  Colours are the standard matplotlib viridis samples.
\pgfplotsset{
  colormap={viridis}{
    rgb=(0.267004,0.004874,0.329415)  % 0.0  dark purple
    rgb=(0.282623,0.140926,0.457517)
    rgb=(0.253935,0.265254,0.529983)
    rgb=(0.206756,0.371758,0.553117)
    rgb=(0.163625,0.471133,0.558148)
    rgb=(0.127568,0.566949,0.550556)  % 0.5  teal
    rgb=(0.134692,0.658636,0.517649)
    rgb=(0.266941,0.748751,0.440573)
    rgb=(0.477504,0.821444,0.318195)
    rgb=(0.741388,0.873449,0.149561)
    rgb=(0.993248,0.906157,0.143936)  % 1.0  yellow
  },
}

% ----- Configuration (always evaluated, even in arXiv/only-names mode) -------
% These control the externalized figure filename and the axis geometry, so they
% must be set regardless of whether we (re)generate the data.
% Number of decoder layers (columns).  Caller may override via \heatmapnlayers.
\ifdefined\heatmapnlayers\else\def\heatmapnlayers{32}\fi
\edef\heatmapmaxidx{\the\numexpr\heatmapnlayers-1\relax}%
% Per-invocation counter, used for unique temp-file names and as a fallback
% cache key.  Incremented once per \input of this file.
\ifdefined\heatmapfilecounter\else\newcount\heatmapfilecounter\fi
\advance\heatmapfilecounter by 1
% Cache key for the externalized figure filename (letters/digits/underscores
% only).  Callers set \heatmapcachekey; fall back to the invocation counter.
\ifdefined\heatmapcachekey\else\edef\heatmapcachekey{\the\heatmapfilecounter}\fi

% When externalization runs in "only graphics" mode (no shell-escape, e.g. arXiv),
% the figure is taken from its cached PDF, so we skip ALL data loading and grid
% generation below.  \heatmaponlynames is defined by main.tex in that case.
\ifdefined\heatmaponlynames\else

% ----- Load data ------------------------------------------------------
\pgfplotstableread[col sep=comma]{\heatmapcsv}\heatmaprawdata

% ----- Reshape (layer,freq) rows into an (x,y,meta) grid --------------
% Each "layer" string is "<type>_<index>", e.g. "gate_proj_31".  We must split
% it into the tensor type (which itself may contain underscores) and the
% trailing numeric index.
%
% (1) Split on the LAST underscore -> \hmtype (e.g. gate_proj) and
%     \hmidx (e.g. 31).
% (2) Map \hmtype to a y row index via a lookup macro; unknown types are
%     skipped.

% --- (1) split on the last underscore --------------------------------------
% \hmsplitlast{<string>} sets \hmtype (everything before the last "_") and
% \hmidx (everything after it).  We append a trailing "_\hmstop" so every real
% segment is followed by "_"; \hmscan then consumes "<seg>_" repeatedly.  While
% the remainder is non-empty the segment belongs to the type prefix; when the
% remainder becomes empty the segment is the trailing numeric index.
% Examples:
%   gate_proj_31 -> \hmtype=gate_proj, \hmidx=31
%   v_proj_3     -> \hmtype=v_proj,    \hmidx=3
\def\hmsplitlast#1{%
  \def\hmtype{}\def\hmidx{}%
  \hmscan#1_\hmstop
}
% Grab "<seg>_"; #1 = seg, #2 = remainder up to \hmstop.
\def\hmscan#1_#2\hmstop{%
  \def\hmremainder{#2}%
  \ifx\hmremainder\empty
    % #1 is the LAST segment -> the numeric index.
    \def\hmidx{#1}%
  \else
    % #1 is part of the type prefix.
    \hmappendtype{#1}%
    \hmscan#2\hmstop
  \fi
}
\def\hmappendtype#1{%
  \ifx\hmtype\empty
    \def\hmtype{#1}%
  \else
    \edef\hmtype{\hmtype_#1}%
  \fi
}

% --- (2) tensor type -> y row index ---------------------------------------
% Lookup table via \csname; \hmrow is set to the row index, or left empty for
% unknown types (which are then skipped).
\expandafter\def\csname hmrow@q_proj\endcsname{0}
\expandafter\def\csname hmrow@k_proj\endcsname{1}
\expandafter\def\csname hmrow@v_proj\endcsname{2}
\expandafter\def\csname hmrow@o_proj\endcsname{3}
\expandafter\def\csname hmrow@gate_proj\endcsname{4}
\expandafter\def\csname hmrow@up_proj\endcsname{5}
\expandafter\def\csname hmrow@down_proj\endcsname{6}
\def\hmlookuprow{%
  \ifcsname hmrow@\hmtype\endcsname
    \edef\hmrow{\csname hmrow@\hmtype\endcsname}%
  \else
    \def\hmrow{}%
  \fi
}

% --- pass 1: store every frequency in a lookup macro ----------------------
% \csname hmval@<type>_<idx>\endcsname = frequency.  This lets us emit the grid
% in a fixed, row-major order below, which is what "matrix plot" requires
% (it positions cells by their order in the table, using mesh/cols + ordering,
% not by the x/y values).  The CSV is sorted by frequency, so we must reorder.
%
% We iterate over the table row indices (0 .. N-1) with a plain \foreach and
% read each cell with \pgfplotstablegetelem, which is robust across
% pgfplotstable versions.
\pgfplotstablegetrowsof{\heatmaprawdata}%
\edef\heatmapnumrows{\pgfplotsretval}%
\begingroup
\foreach \hmrowidx in {0,...,\the\numexpr\heatmapnumrows-1\relax}{%
  \pgfplotstablegetelem{\hmrowidx}{layer}\of\heatmaprawdata%
  \let\hmcell\pgfplotsretval
  \pgfplotstablegetelem{\hmrowidx}{high_precision_frequency}\of\heatmaprawdata%
  \let\hmval\pgfplotsretval
  \expandafter\hmsplitlast\expandafter{\hmcell}%
  \hmlookuprow
  \ifx\hmrow\empty\else
    \expandafter\xdef\csname hmval@\hmtype _\hmidx\endcsname{\hmval}%
  \fi
}%
\endgroup

% --- pass 2: write the grid to a temp file in row-major order -------------
% We iterate the tensor types paired with their row index using TikZ's
% \foreach "value/label" syntax, and for each type iterate the layer indices
% 0..\heatmapmaxidx.  Missing cells (which do not occur for these CSVs) default
% to 0.  The rows are written to a real file with one "<x> <y> <meta>" line
% each; this avoids all inline/"row sep=crcr" restrictions and is read back as
% an ordinary whitespace-separated table.
% Declare the write stream only once (this file may be \input several times).
\ifdefined\heatmapout\else\newwrite\heatmapout\fi
% Unique temp-file name per invocation so multiple heatmaps in one document do
% not clobber each other's data.
\edef\heatmapdatafile{\jobname.heatmapgrid\the\heatmapfilecounter.dat}%
\immediate\openout\heatmapout=\heatmapdatafile
\immediate\write\heatmapout{x y meta}%
\begingroup
\foreach \hmt/\hmrownum in {%
    q_proj/0,k_proj/1,v_proj/2,o_proj/3,gate_proj/4,up_proj/5,down_proj/6}{%
  \foreach \hmi in {0,...,\heatmapmaxidx}{%
    \ifcsname hmval@\hmt _\hmi\endcsname
      \edef\hmcellval{\csname hmval@\hmt _\hmi\endcsname}%
    \else
      \def\hmcellval{0}%
    \fi
    \immediate\write\heatmapout{\hmi\space\hmrownum\space\hmcellval}%
  }%
}
\endgroup
\immediate\closeout\heatmapout

% Read the freshly written grid back as a normal table.
\pgfplotstableread{\heatmapdatafile}\heatmapgridtable

\fi % end \ifdefined\heatmaponlynames\else  (data build skipped for cached mode)

% ----- Figure ---------------------------------------------------------
% Caching (TikZ externalization): give this figure a stable, readable cache
% name derived from the title, and declare the source CSV as a dependency so
% the cached PDF is regenerated whenever the underlying data changes.
% Both are no-ops when externalization is disabled.
\ifdefined\tikzsetnextfilename
  \edef\heatmapextname{frequency_heatmap_\heatmapcachekey}%
  \expandafter\tikzsetnextfilename\expandafter{\heatmapextname}%
\fi
\ifdefined\tikzpicturedependsonfile
  \expandafter\tikzpicturedependsonfile\expandafter{\heatmapcsv}%
\fi
\begin{tikzpicture}
  \begin{axis}[
      title={\heatmaptitle},
      title style={font=\small\bfseries},
      width=0.95\textwidth, height=0.42\textwidth,
      enlargelimits=false, axis on top,
      xlabel={decoder layer index (0 = first, \heatmapmaxidx\ = last)},
      label style={font=\scriptsize},
      tick label style={font=\tiny},
      xmin=-0.5, xmax=\heatmapmaxidx.5,
      ymin=-0.5, ymax=6.5,
      xtick={0,2,...,\heatmapmaxidx},
      ytick={0,1,2,3,4,5,6},
      yticklabels={%
        \texttt{q\_proj}, \texttt{k\_proj}, \texttt{v\_proj},
        \texttt{o\_proj}, \texttt{gate\_proj}, \texttt{up\_proj},
        \texttt{down\_proj}},
      y dir=reverse,                % q_proj on top (like the reference figure)
      tick align=outside, tick pos=left,
      colormap name=viridis,
      colorbar,
      point meta min=0, point meta max=1,
      colorbar style={
        ylabel={high-precision frequency},
        ylabel style={font=\scriptsize},
        ytick={0,0.2,0.4,0.6,0.8,1.0},
        tick label style={font=\tiny},
      },
    ]
    \addplot[
      matrix plot*,
      mesh/cols=\heatmapnlayers, % layer indices per row
      mesh/rows=7,               % 7 tensor-type rows
      mesh/ordering=x varies,    % x (layer index) changes fastest — matches emit order
      point meta=explicit,
    ] table [x=x, y=y, meta=meta] {\heatmapgridtable};
  \end{axis}
\end{tikzpicture}%
% Reset per-figure parameters so each invocation must set them explicitly and
% stale values do not leak into a subsequent \input (e.g. a different model with
% a different layer count or cache key).
\let\heatmapcachekey\undefined
\let\heatmapnlayers\undefined

